PECC: Problem Extraction and Coding Challenges

Recent advancements in large language models (LLMs) have showcased their exceptional abilities across various tasks, such as code generation, problem-solving and reasoning. Existing benchmarks evaluate tasks in isolation, yet the extent to which LLMs can understand prose-style tasks, identify the underlying problems, and then generate appropriate code solutions is still unexplored. Addressing this gap, we introduce PECC, a novel benchmark derived from Advent Of Code (AoC) challenges and Project Euler, including 2396 problems. Unlike conventional benchmarks, PECC requires LLMs to interpret narrative-embedded problems, extract requirements, and generate executable code. A key feature of our dataset is the complexity added by natural language prompting in chat-based evaluations, mirroring real-world instruction ambiguities. Results show varying model performance between narrative and neutral problems, with specific challenges in the Euler math-based subset with GPT-3.5-Turbo passing 50% of the AoC challenges and only 8% on the Euler problems. By probing the limits of LLMs' capabilities, our benchmark provides a framework to monitor and assess the subsequent progress of LLMs as a universal problem solver.

==> prompt_strucutre.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1.0, 0.94, 0.96}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{pink},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
}

\lstset{style=mystyle}

\lstset{emph={%  
    System, User, AI, OutputPrinter%
    },emphstyle={\color{red}\bfseries\underbar}%
}%

\subsection{Prompt Structure}
\begin{lstlisting}
System: You are a code generator and given a programming task. A file with the input to your program is called 'input.txt'. Generate only directly executable python code.
\end{lstlisting}

\begin{lstlisting}
User: Given a list of comma seperated integers, like `1,2,3`. Calculate the some of all integers. The sum of `1,2,3` would be `6`.
\end{lstlisting}

\begin{lstlisting}
AI: def list_sum(lst)):
        return sum(lst)
    
    file_name = "{input_file_name}"
    with open(file_name, "r") as f:
        lst = eval(f.read())
    
    print("Result: " + list_sum(lst))
\end{lstlisting}

\begin{lstlisting}
System: Here is the output of your program: 'Result: 15'. Please only return the resulting number or text and nothing else.
\end{lstlisting}

\begin{lstlisting}
AI: 15
\end{lstlisting}

\begin{lstlisting}
System: You are a code generator and given a second part of a programming task. A file with the input to your program is called 'input.txt'. Generate only directly executable python code.
\end{lstlisting}

\begin{lstlisting}
User: Based on the result of the summing function, calculate the next prime number.
\end{lstlisting}

